ES-HPC-MPC: Exponentially Stable Hybrid Perception Constrained MPC for Quadrotor with Suspended Payloads

Aerial transportation using quadrotors with cable-suspended payloads holds great potential for applications in disaster response, logistics, and infrastructure maintenance. However, their hybrid and underactuated dynamics pose significant control and perception challenges. Traditional approaches often assume a taut cable condition, limiting their effectiveness in real-world applications where slack-to-taut transitions occur due to disturbances. We introduce ES-HPC-MPC, a model predictive control framework that enforces exponential stability and perception-constrained control under hybrid dynamics. Our method leverages Exponentially Stabilizing Control Lyapunov Functions (ES-CLFs) to enforce stability during the tasks and Control Barrier Functions (CBFs) to maintain the payload within the onboard camera's field of view (FoV). We validate our method through both simulation and real-world experiments, demonstrating stable trajectory tracking and reliable payload perception. We validate that our method maintains stability and satisfies perception constraints while tracking dynamically infeasible trajectories and when the system is subjected to hybrid mode transitions caused by unexpected disturbances.

==> sections/archived.tex <==
highlight the necessity of a hybrid controller, 


% \begin{figure}[htbp]
%     \centering
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=800 0 800 0, clip]{figures/nonhybrid_hover_gripper_gif/0.PNG} % Path to your image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=800 0 800 0, clip]{figures/nonhybrid_hover_gripper_gif/1.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=800 0 800 0, clip]{figures/nonhybrid_hover_gripper_gif/2.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=800 0 800 0, clip]{figures/nonhybrid_hover_gripper_gif/3.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=800 0 800 0, clip]{figures/nonhybrid_hover_gripper_gif/4.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=800 0 800 0, clip]{figures/nonhybrid_hover_gripper_gif/5.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=800 0 800 0, clip]{figures/nonhybrid_hover_gripper_gif/6.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/plots_larger_font_v2/july_1_3_nohybrid_hover_manual_vertical_move.pdf}
%     \end{minipage}
%     \hfill
%     \caption{Non-Hybrid controller during a slack-taut transition in a hover scenario. The controller incorrectly commands the robot to move towards the payload during the slack state due to $z$ error in the desired payload position. We release the payload at $t=1.2$ to prevent a crash.}
%     \label{fig:non_hybrid_hover_gif}
% \end{figure}
% 
% \begin{figure}[htbp]
%     \centering
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=200 0 200 0, clip]{figures/hybrid_hover_manual_gripper_gif/0.PNG} % Path to your image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=200 0 200 0, clip]{figures/hybrid_hover_manual_gripper_gif/1.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=200 0 200 0, clip]{figures/hybrid_hover_manual_gripper_gif/2.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=200 0 200 0, clip]{figures/hybrid_hover_manual_gripper_gif/3.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=200 0 200 0, clip]{figures/hybrid_hover_manual_gripper_gif/4.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=200 0 200 0, clip]{figures/hybrid_hover_manual_gripper_gif/5.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.13\columnwidth}
%         \centering
%         \includegraphics[width=\textwidth, trim=200 0 200 0, clip]{figures/hybrid_hover_manual_gripper_gif/6.PNG} % image
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/plots_larger_font_v2/july_1_4_hybrid_hover_manual_vertical_move.pdf}
%     \end{minipage}
%     \caption{Hybrid controller during a slack-taut transition in a hover scenario. The robot maintains its position and is unaffected by the payload movement.}
%     \label{fig:hybrid_hover_gif}
% \end{figure}

\begin{figure*}
    \begin{minipage}[b]{1.5\columnwidth}
    \hspace{-10pt}
    \includegraphics[width=\textwidth, trim=100 250 100 300, clip]{figures/system_overview.pd}
    \end{minipage}
    \begin{minipage}[b]{0.55\columnwidth}
        \centering
        \includegraphics[width=\textwidth, trim=400 250 400 200, clip]{figures/system_convention_frames_2.pdf} \label{fig:figure1}
    \end{minipage}    
    \caption{(Left) The system architecture describing the flow of information through the various components of our pipeline. (Right) System Frame Convention}
    \label{fig:sys_overview}
\end{figure*}



%\begin{itemize}
%    \item We propose a novel Model Predictive Control approach enhanced with ES-CLFs and CBFs. This formulation stabilizes hybrid dynamics in quadrotor systems with cable-suspended payloads while ensuring safety perception by maintaining the payload within the camera’s FOV.
%    
%    \item  We address the stability challenges posed by hybrid dynamics by incorporating dynamically updated ES-CLFs for payload trajectory tracking and CBFs for payload visibility. These functions ensure that the controller contracts
%faster and enforce safety properties during cable transitions, ensuring consistent trajectory tracking and human-payload interactions.
%    
%    \item We validate the framework through simulations and real-world experiments using only on-board sensors. The results demonstrate stable trajectory tracking and robust performance during slack-to-taut transitions, while ensuring the payload remains within the camera’s FOV, even during human manipulation.
%
%\end{itemize}


\subsection{Exponentially Stabilizing Control Lyapunov Functions}
%We will begin by reviewing ES-CLFs and exploring their role in synthesizing controllers that ensure stability.
A continuously differentiable function $V(\cdot): \mathcal{X} \rightarrow \mathbb{R}_{\geq 0}$ is an ES-CLF for \eqref{eq:hybrid_dynamics_control_affine} if there exists $\mathbf{C}_1, \mathbf{C}_2,  \mathbf{C}_3 > 0$ such that
 \begin{equation}
\|\vecx\|^{2}_{\mathbf{C}_1}  \leq V(\vecx) \leq \|\vecx\|^{2}_{\mathbf{C}_2} 
\label{eq:exponentially_lyapunov}
\end{equation}
 \begin{equation}
 \inf_{\vecu \in \mathcal{U}} \dot{V}(\vecx, \vecu) \leq -\|\vecx\|^{2}_{\mathbf{C}_3}
\label{eq:exponentially_lyapunov_dot}
\end{equation}
The existence of \(V(\vecx)\) is both a necessary and sufficient condition for the existence of a state-feedback controller.
%\(\mathbf{k}_{clf}(\cdot): \mathcal{X} \rightarrow \mathcal{U}\), that guarantees global exponential stability. This ensures that the state vector \(\vecx\) converges exponentially to the equilibrium, with the convergence rate determined by \(\mathbf{C}_3\) \cite{8796030}. 
The set of stabilizing controllers for all \(\vecx \in \mathcal{X}\) can be defined as:
 \begin{equation}
\mathcal{U}_{clf}(\vecx) = \{\vecu \in \mathcal{U}~|~\dot{V}(\vecx, \vecu) \leq -\|\vecx\|^{2}_{\mathbf{C}_3}\}
\label{eq:exponentially_set}
\end{equation}
where $\dot{V}(\vecx, \vecu)$ can be expressed in terms of the dynamics as $\dot{V}(\vecx, \vecu) = \frac{\partial V(\vecx)}{\partial \vecx}(\mathbf{f}(\vecx, s) + \mathbf{g}(\vecx, s) \vecu)$.
% \begin{equation}
%\dot{V}(\vecx, \vecu) = \frac{\partial V(\vecx)}{\partial \vecx}(\mathbf{f}(\vecx, s) + \mathbf{g}(\vecx, s) \vecu)
%\end{equation}
Eq. \eqref{eq:exponentially_set} facilitates the formulation of optimization-based controllers with desirable characteristics through quadratic programming (QP) \cite{7079382, 6709752} and MPC formulations \cite{Grandia2020}.



\subsection{Control Barrier Functions}
 We can define \(\mathcal{H}\) as the superlevel set of a continuously differentiable function $h(\cdot): \mathcal{X} \rightarrow \mathbb{R}$, such that

\begin{equation}
\begin{aligned}
\mathcal{H} &= \{\vecx \in \mathcal{X} \mid h(\vecx) \geq 0\} \\
%\partial\mathcal{H} &= \{\vecx \in \mathcal{X} \mid h(\vecx) = 0\}
%\\
%\textrm{Int}(\mathcal{H}) &= \{\vecx \in \mathcal{X} \mid h(\vecx) > 0\}
\end{aligned}
\label{eq:barrier_set}
\end{equation}
The function \(h(\cdot)\) is defined as a CBF for all \(\vecx \in \mathcal{X}\) if there exists an extended class \(\mathcal{K}_{\infty}\) function %\(\alpha\) 
for \eqref{eq:hybrid_dynamics_control_affine}, satisfying the following condition:
 \begin{equation}
  \sup_{\vecu \in \mathcal{U}} \dot{h}(\vecx, \vecu) \geq - \alpha(h(\vecx)) 
\label{eq:barrier_condition}
\end{equation}
%The existence of \(h(\vecx)\) is sufficient to guarantee that a controller \(\mathbf{k}_{cbf}(\cdot): \mathcal{X} \rightarrow \mathcal{U}\) renders the set \(\mathcal{H}\) safe. 
Therefore, safety can be ensured through a CBF, which defines the set of controllers that render \(\mathcal{H}\) safe, as follows:
 \begin{equation}
\mathcal{U}_{cbf}(\vecx) = \{\vecu \in \mathcal{U}~|~\dot{h}(\vecx, \vecu)  \geq - \alpha(h(\vecx)) \}
\label{eq:barrier_set_condition}
\end{equation}
Eq.~\eqref{eq:barrier_set_condition} allows the formulation of controllers  with safety guarantees using QPs \cite{8796030} and MPC approaches \cite{9483029}.
%$$
%\bm{\eta}^{\camerafsmall} = \hamiltomminus(\hamiltomplus(\cameraquat)\loadposc + \hamiltomminus(\cameraquat) \camerapos)
%$$
%$$
%\bm{\mu}^{\camerafsmall} = \hamiltomplus(\hamiltomminus(\cameraquat^{*})\loadposc + \hamiltomplus(\cameraquat^{*}) \camerapos)
%$$


if $k_q > \frac{c_1 k^{2}_{vq} +2 c_1 k_{vq} - c^{2}_1}{\loadquad(4(k_{vq} - c_1)-1)}$ and $k_{vq} > c_1 +\frac{1}{4}$, then 
 and if  $k_{R} > \frac{c_2 k^{2}_{\omega}}{\lambda_m(4(k_{\omega} -1/2 c_2) -1)}$ and $k_\omega > \frac{1}{2} c_2 + \frac{1}{4}$,

 if $k_l > \frac{c_3 k^{2}_{vl} +2 c_3 k_{vl} - c^{2}_3}{\loadmass (4(k_{vl} - c_3)-1)}$ and $k_{vl} > c_3 +\frac{1}{4}$, $V_{\loadpos{}}$, then  $ V_{\loadpos{}}$ can be defined  bounded by Cauchy-Schwartz inequality as follows:



 % Quadrotors with cable-suspended loads offer significant advantages in autonomous aerial transportation due to their agility, energy efficiency, and mechanical simplicity.  However, they are underactuated, hybrid and non-linear and rely on limited on-board computational resources for their control and perception algorithms. Consequently, deploying them in real-world environments poses substantial challenges in ensuring stable control and continuous state estimation.
% %In response, we propose a Model Predictive Control (MPC) framework enhanced by Exponentially Stabilizing Control Lyapunov Functions (ES-CLFs) and Control Barrier Functions (CBFs). This approach ensures closed-loop stability under hybrid dynamics and maintains payload visibility by keeping the payload within the camera field of view (FOV),  thereby enabling accurate full-state estimation via an Extended Kalman Filter (EKF).
% To address these challenges, we propose an Exponentially Stable Hybrid Perception-Constrained MPC (ES-HPC-MPC) for quadrotors with suspended loads. This approach ensures stability under hybrid dynamics using Exponentially Stabilizing Control Lyapunov Functions (ES-CLFs) and maintains the payload in the camera's field of view (FOV) via Control Barrier Functions (CBFs). 
% %This framework thereby enables accurate full-state estimation through an Extended Kalman Filter (EKF).
% We validate the proposed control framework through both simulation and real-world experiments. The results demonstrate stable trajectory tracking, even during slack-to-taut transitions of the cable. Furthermore, the perception CBF guarantees that the payload remains within the robot’s camera FOV, allowing for safe operation under unexpected hybrid mode transitions.

% version 2 
%Quadrotors with cable-suspended loads are promising robot alternatives for autonomous aerial transportation due to their agility and mechanical simplicity. However, deploying them in real-world environments remains an unsolved problem due to control and state estimation challenges that arise from the system's under-actuated and hybrid dynamics. Our proposed method, ES-HPC-MPC, ensures stability under hybrid dynamics using Exponentially Stabilizing Control Lyapunov Functions (ES-CLFs) and maintains the payload in the camera's field of view (FOV) via Control Barrier Functions (CBFs). We validate the proposed control framework through both simulation and real-world experiments. The results demonstrate stable trajectory tracking and reliable perception awareness in both simulation and real-world settings. We experimentally validate that our method maintains stability and satisfies perception constraints while tracking dynamically infeasible trajectories and when the system is subjected to hybrid mode transitions caused by unexpected disturbances. 


%We integrate these equations into our MPC method by defining the OCP's running and terminal cost to represent the Lyapunov function in Eq.\eqref{eq:lyapunov_translation} and define $\mathbf{g}_{clf}$ to represent the constraint in Eq.\eqref{eq:lyapunov_inequality_dot}.





%We proposed a novel formulation of a trajectory tracking metric using ES-CLFs for a hybrid quadrotor with suspended payload system. We ensure exponential controller stability under both slack and taut cable states and gurantee stability by integrating the CLF into our proposed MPC framework 

%We propose a novel formulation of perception awareness using CBFs to ensure continuous state estimation of the hybrid system during both slack and taut modes. We guarantee perception awareness by usingconstraining the system to satisfy second order CBF constraints


%We propose a novel formulation of trajectory tracking using Exponentially Stabilizing Control Lyapunov Functions (ES-CLFs), and address perception awareness using Control Barrier Functions (CBFs), for a hybrid quadrotor with suspended payload system. 



%Numerous works have been proposed to address the challenges associated with controlling quadrotor cable-suspended load systems \cite{GUERREROSANCHEZ2017433}. These approaches often minimize the swing angle of the payload, constraining its range of motion and limiting its ability to perform agile maneuvers. 

%In recent years, quadrotors equipped with suspended payloads have become increasingly important in logistics, transportation, and disaster relief \cite{water_sampling, Masone2021SharedPayload, Jimenez-Cano2022PreciseTechniques}. Researchers have developed advanced trajectory tracking strategies based on non-linear geometric control \cite{guanrui2021ral, 7892030} and MPC \cite{10243043, 10156031, 10341785, 9007450}. Despite these advances, hybrid dynamics, due to slack-to-taut cable transitions, remains a critical challenge, which if neglected can lead to failures in both control and full-state estimation. Furthermore, current methods lack mechanisms to ensure that the payload consistently remains within the camera’s FOV, which is crucial for maintaining reliable and accurate state estimation of the load. \cite{sarah2018icra}.


%% MPC Section
%In this section, we present the ES-HPC-MPC for quadrotors with suspended payloads. The cost functions and inequality constraints based on ES-CLF are dynamically updated to adapt based on whether the cable is taut or slack. The ES-CLF is designed to reduce translational and rotational errors to ensure accurate trajectory tracking, while the CBF is constructed to ensure that the payload remains in the camera's FOV. Fig. \ref{fig:sys_overview} illustrates the system overview of our solution.

% In this section, we introduce the \textbf{E}xponentially \textbf{S}table \textbf{H}ybrid \textbf{P}erception-\textbf{C}onstrained \textbf{M}odel \textbf{P}redictive \textbf{C}ontrol (\textbf{ES-HPC-MPC}) for quadrotors transporting suspended payloads. Our method not only considers the hybrid system dynamics but also ensures stable trajectory tracking through ES-CLFs and perception safety through CBFs. The ES-CLF is designed to guarantee exponential stability by minimizing trajectory tracking errors, while the proposed CBF simultaneously enforces the payload's visibility within the camera’s FOV. We highlight that our method is designed and experimentally validated to work not only in each hybrid mode, but also during mode transitions caused by unexpected disturbances. This hybrid-aware formulation enables the controller to achieve stability and safety guarantees, enhancing the system’s resilience to unanticipated disturbances and improving onboard state estimation reliability. Fig. \ref{fig:sys_overview} provides an overview of the system architecture.


% In this paper, we design the terminal and running costs based on an ES-CLF, ensuring exponential convergence of trajectory tracking errors as detailed in Section. \ref{sec:Dynamically Update ES-CLF}. Furthermore, we impose an inequality constraint on the time derivative of the ES-CLF through the inequality \eqref{eq:inequality_constraint_clf}. And we show the details of this inequality in Section~\ref{sec:Dynamically Update ES-CLF}. Finally, we also develop a CBF to maintain the payload within the camera’s field of view, as denoted by $\mathbf{g}_{cbf}(\vecx, \vecu, s)$ shown in Section~\ref{sec:Safe Perception Control Barrier Function}. In the following sections, we present the detailed formulations of these costs and constraints.


%Finally, we must satisfy the following constraint on $\dot{V}_{\robotpos{}}$
% The existence of a stabilizing controller implies that $\dot{V}_{\robotpos{}}$ is bounded by the following expression:


% By ensuring that the conditions specified in \eqref{eq:lyapunov_translation_quad_inequality} and \eqref{eq:lyapunov_translation_quad_inequality_dot} are satisfied, it is established that \(V_{\robotpos{}}\) remains bounded and \(\dot{V}_{\robotpos{}}\) is negative. Therefore, \(V_{\robotpos{}}\) serves as an appropriate ES-CLF for the translational dynamics of the quadrotor, guaranteeing global exponential convergence.

% By ensuring that \eqref{eq:lyapunov_translation_load_inequality} and \eqref{eq:lyapunov_translation_load_inequality_dot} are satisfied, \(V_{\loadpos{}}\) is bounded, while \(\dot{V}_{\loadpos{}}\) is negative. Therefore, \(V_{\loadpos{}}\) can be defined as an ES-CLF for the payload dynamics.

%By combining \eqref{eq:lyapunov_translation_quad_inequality}, \eqref{eq:lyapunov_rotational_quad_inequality}, and \eqref{eq:lyapunov_translation_load_inequality}, we can bound the control Lyapunov function of the whole system $V$ as follows:

% More details regarding $\mathbf{z}$, $\shortunderline{\mathbf{Q}}$ and $\bar{\mathbf{Q}}$  are provided in Section~\ref{Quadrotor ES-CLF} and \ref{Payload ES-CLF}.

% The Lie derivative can be used to compute \(\dot{V}(\vecx, \vecx_{ref}, \vecu)\). 
% By guaranteeing that the definitions in  \eqref{eq:lyapunov_inequality} and \eqref{eq:lyapunov_inequality_dot} are satisfied, we can ensure that \(V\) is bounded and \(\dot{V}\) is negative semi-definite. Consequently, \(V\) is an ES-CLF for the hybrid dynamics of the quadrotor with a cable-suspended load. The formulation detailed in \eqref{eq:lyapunov_translation} has been integrated into the MPC as both a running and terminal cost. Furthermore, the inequality in \eqref{eq:lyapunov_inequality_dot} has been incorporated as a constraint.

%The formulation in Eq. \eqref{eq:barrier_set_condition_perception} is included as a constraint within the MPC framework in Eq. \eqref{eq:MPC} to ensure safe perception.
%We highlight that unlike \cite{mrunal2025hpampc}, the modification of
%the eigenvalues of $\mathbf{K}$ changes the shape of the ellipse, making it adequate for the asymmetric resolution of the camera $1280 \times 720$. This formulation allows our method to exploit the asymmetric camera image during certain trajectories, as shown in Section \ref{subsubsec:exp_infeasible_traj}.

% \begin{equation}
% \underbrace{-\|\loadposc\|^{2}_{\mathbf{K}} + r^{2}_{max}}_{h(\vecx)} \geq 0
% \label{eq:barrier_function_perception}
% \end{equation}
% where $\mathbf{K} > 0$ characterizes the shape of the ellipse and $r_{max}$ represents the maximum radius of the safety set within the camera frame. The function $h(\vecx)$ is a CBF if we can satisfy the following condition:
% \begin{equation}
% \dot{h}(\vecx, \vecu)  \geq - \alpha h(\vecx) 
% \label{eq:barrier_set_condition_perception}
% \end{equation}
% where $\dot{h}(\vecx, \vecu)$ is derived using Lie derivatives, and $\alpha > 0$ is a scalar. The formulation in Eq. \eqref{eq:barrier_set_condition_perception} is included as a constraint within the MPC framework in Eq. \eqref{eq:MPC} to ensure safe perception.



%% Restuls 
%This section presents the simulation results comparing our method ES-HPC-MPC with the HPA-MPC (baseline) in \cite{mrunal2024hpampc}. We analyze the tracking performance of both controllers under 20 Lissajous trajectories with speed ranging from $1.5$ m/s to $3.5$ m/s. We also evaluate the controllers' performance under model mismatch or random disturbances that cause hybrid mode transitions. We report the Root Mean Squared Error (RMSE) of the trajectory tracking and perception constraints violation rates of the two methods in Table \ref{table_simulation}. 

%% Real world
% This section details the evaluation of our MPC with Perception and Stability Guarantees. We demonstrate the advantages of our formulation through experiments that involve trajectory tracking with slack-to-taut transitions induced by unexpected disturbances. Through these experiments, we establish that our method exhibits stable trajectory tracking and robust performance during moded transitions while ensuring that the payload remains within the camera's FOV.


% We showcase the effectiveness of our approach in maintaining the payload within the system's FOV under high-acceleration scenarios. We demonstrate that our method is able to both maintain the load within the camera's FOV, and rapidly converge to the desired position set-point by exploiting the asymmetric camera resolution.

% Finally, we verify that our approach ensures that the quadrotor maintains the payload within its FOV during trajectory tracking tasks and during hybrid mode transitions triggered by human-payload manipulation tasks.


% Here we present the trajectory tracking results under the application of an unexpected vertical impulse force applied to the payload during trajectory tracking. Snapshots of the experiment are shown in Fig. \ref{fig:manipulation_trajectory}a. During the trajectory execution, random human-payload disturbances push the payload upward, causing the cable to go slack and potentially move the load outside the camera's FOV.

% We show that our method can exploit the asymmetric camera resolution to maintain the load in the camera's FOV while ensuring quadrotor stability.

% Snapshots of the robot's movements during this experiment are shown in Fig.
% \ref{fig:point_to_point}a. The control error metrics presented in Fig. \ref{fig:point_to_point}b, highlight a significant position error of the payload, reaching up to \(1~[m]\) at a specific instant, which generates substantial accelerations. Despite these challenges, our formulation successfully ensures that the payload remains within the FOV (see Fig. \ref{fig:point_to_point}d) by adjusting the angular velocity \(\omega_z\), as depicted in Fig. \ref{fig:point_to_point}c. This adjustment shifts the payload to the maximum width of the image, which guarantees the visibility along the experiment. Finally, Fig. \ref{fig:point_to_point}e displays the images captured by the camera, illustrating how our formulation dynamically modifies the system's orientation to maintain the payload within the maximum width of the camera.

==> sections/geom_control_and_traj_gen.tex <==
\section{Geometric Control and Trajectory Generation} 
\subsection{Nominal Geometric Controller}
We provide a brief overview of the well known geometric controller for a quadrotor attached to a point-mass suspended payload developed by \cite{sreenath2013cdc} and a simple payload trajectory generation scheme. Given a desired payload trajectory, the desired force acting on the payload is
\begin{align}
\vecF_{des} = &~\prths{m+\loadmass}\prths{\matK_{p}\vece_{\loadpos}+\matK_{d}\vece_{\loadvel}+\matK_{i}\int_0^t\vece_{\loadpos}d\tau}\nonumber\\
&~+\prths{m+\loadmass}\prths{\loadaccdes + \vecg}+ml\prths{\cabledotvec{}\cdot\cabledotvec{}}\cablevec{}, \label{eq:control-single-cable-plpos-control}
\end{align}
where $\matK_{p},\matK_{d},\matK_{i}\in\realnum{3\times3}$ are diagonal gain matrices and $\vece_{\loadpos},\vece_{\loadvel}\in\realnum{3}$ are the payload position and velocity errors defined as
\begin{equation}
\begin{split}
\vece_{\loadpos} = \loadposdes - \loadpos,\\
\vece_{\loadvel} = \loadveldes - \loadvel,~\label{eq:payload-pos-error}
\end{split}
\end{equation}
Since the desired force $\vecF_{des}$ is exerted by the tension cable, it defines the desired tension force vector. Hence the desired tension direction $\cablevec{des}$ can be obtained as
\begin{equation}
 \cablevec{des} = \frac{\vecF_{des}}{\twonorm{\vecF_{des}}}. 
\end{equation}
The thrust $f$ and moment $\matM$ acting on the quadrotor are
\begin{align}
f =& \vecF\cdot\robotrot{}\axis{3}{}\\
\vecF =&\cablevec{}\cablevec{}^\top\vecF_{des}-ml\cablevec{}\times\prths{\matK_{\cablevec{}}\vece_{\cablevec{}}+\matK_{\cablevel{}}\vece_{\cablevel{}}+\prths{\cablevec{}\cdot\cablevel{des}}\cabledotvec{}}\nonumber\\
~&+ml\cablevec{}\times\prths{\cablevec{des}\times\cableddotvec{des}},\label{eq:control-single-cable-qdthrust-control}
\end{align}
\begin{equation}
\begin{split}
\mathbf{M} =&~\matK_{R}\vece_{R} + \matK_{\Omega}\vece_{\Omega} + \robotangvel{}\times\inertia\robotangvel{}\\
&-\inertia\prths{\hat{\robotangvel{}}\robotrot{}^{\top}\robotrot{des}\robotangvel{des}-\robotrot{}^{\top}\robotrot{des}\dot{\robotangvel{}}_{des}},\label{eq:control-single-cable-qdatt-control}
\end{split}
\end{equation}
where $\matK_{R},\matK_{\Omega},\matK_{\cablevec{}},\matK_{\cablevel{}}\in\realnum{3\times3}$ are diagonal gain matrices, $\vece_{R} , \vece_{\Omega}\in\realnum{3}$ are quadrotor's orientation, angular velocity errors defined as
\begin{equation}
\begin{split}
\vece_{\robotrot{}} &= \half\prths{\robotrot{}^{\top}\robotrot{des}-\robotrot{des}^{\top}\robotrot{}}^{\vee}, \\
\vece_{\robotangvel{}} &=  \robotrot{}^{\top}\robotrot{des}\robotangvel{des} - \robotangvel{},\label{eq:robot-angular-error}
\end{split}
\end{equation}
and $ \vece_{\cablevec{}}, \vece_{\cablevel{}}\in\realnum{3}$ are cable direction, cable velocity errors defined as
\begin{equation}
\vece_{\cablevec{}}= \cablevec{des} \times\cablevec{},~
\vece_{\cablevel{}} = \cablevel{} + \cablevec{}\times
\cablevec{}\times\cablevel{des}.\label{eq:cable-error}
\end{equation}

\subsection{Trajectory Generation}
We validate our NMPC method to track lissajous payload trajectories that are generated using the following equations
\begin{equation}
\loadposdes(t) = \begin{bmatrix}
    a\sin(t)&b\sin(nt + \phi)&c\sin(mt) + \psi    \label{eq:lissajous_traj_eq}
\end{bmatrix}^\top
\end{equation}
where $n,m$ control the relative periods of $x,y,z$ motions and $a,b$ and $c$ their relative amplitudes. By differentiating \eqref{eq:lissajous_traj_eq}, we obtain $\loadveldes(t)$ and $\loadaccdes(t)$. \\

As we will see in section x.x, it will be useful to know the nominal $\robotdes(t)$ and $\matR_{des} (t)$, which can be calculated using the system's differential flatness properties as shown in \cite{sreenath2013geometric}.

# talk about angular rates
